Resource Efficient Isolation Mechanisms in Mixed-Criticality Scheduling

Mixed-criticality real-time scheduling has been developed to improve resource utilization while guaranteeing safe execution of critical applications. These studies use optimistic resource reservation for all the applications to improve utilization, but prioritize critical applications when the reservations become insufficient at runtime. Many of them however share an impractical assumption that all the critical applications will simultaneously demand additional resources. As a consequence, they under-utilize resources by penalizing all the low-criticality applications. In this paper we overcome this shortcoming using a novel mechanism that comprises a parameter to model the expected number of critical applications simultaneously demanding more resources, and an execution strategy based on the parameter to improve resource utilization. Since most mixed-criticality systems in practice are component-based, we design our mechanism such that the component boundaries provide the isolation necessary to support the execution of low-criticality applications, and at the same time protect the critical ones. We also develop schedulability tests for the proposed mechanism under both a flat as well as a hierarchical scheduling framework. Finally, through simulations, we compare the performance of the proposed approach with existing studies in terms of schedulability and the capability to support low-criticality applications.

==> code.tex <==
\definecolor{light-gray}{gray}{0.95}
\lstset{
	% Basic design
	backgroundcolor=\color{light-gray},
	basicstyle={\scriptsize\ttfamily},   
	frame=l,
	% Line numbers
	xleftmargin={0.75cm},
	numbers=left,
	stepnumber=1,
	firstnumber=1,
	numberfirstline=true,
	% Code design
	identifierstyle=\color{black},
	keywordstyle=\color{blue}\bfseries,
	ndkeywordstyle=\color{greenCode}\bfseries,
	stringstyle=\color{ocherCode}\ttfamily,
	commentstyle=\color{darkgray}\ttfamily,
	% Code
	language={C},
	tabsize=3,
	showtabs=false,
	showspaces=false,
	showstringspaces=false,
	extendedchars=true,
	breaklines=true
}

%\begin{table}[!h]
%	\centering
%	\caption{Compute Kernel Code Descriptions}
%	\label{code.tbl}
%	\begin{tabular}{l}
%	    \toprule
%		\multicolumn{1}{c}{(a) C description}  \\%&\multicolumn{1}{c}{(b) DFG description} \\ % Assembly with Loopback Optimization
%	    \midrule
%		%    \hspace{-0.2in}
%		\begin{lstlisting}
%#define SQR(x) ((x)*(x))
%for(int i=0;i<64;i++)
%	for(int j=1;j<63;j++)
%		for (int k=1;k<63;k++)
%			b[i][j][k] =
%				SQR(a[i][j][k] - a[i][j][k-1]) +
%				SQR(a[i][j][k] - a[i][j][k+1]) +
%				SQR(a[i][j][k] - a[i][j-1][k]) +
%				SQR(a[i][j][k] - a[i][j+1][k]);
%
%		\end{lstlisting}
%		
%		\\
%		\\
%		\toprule
%		\multicolumn{1}{c}{(b) Data Flow Graph}  \\
%		\midrule
%		%    \hspace{-0.2in}
%		%\hfill
%	\begin{tikzpicture}[>=latex',line join=bevel, scale = 0.4]
%	\centering	
%	%\small
%	\tiny
%	\node (N12) at (50.797bp,234.0bp) [draw=black,ellipse] {sqr\_N12};
%	\node (N13) at (152.8bp,162.0bp) [draw=black,ellipse] {add\_N13};
%	\node (N10) at (258.8bp,306.0bp) [draw=black,ellipse] {sub\_N10};
%	\node (N11) at (152.8bp,306.0bp) [draw=black,ellipse] {sub\_N11};
%	\node (N16) at (258.8bp,234.0bp) [draw=black,ellipse] {sqr\_N16};
%	\node (N17) at (205.8bp,18.0bp) [draw=black,ellipse] {O0\_N17};
%	\node (N14) at (258.8bp,162.0bp) [draw=black,ellipse] {add\_N14};
%	\node (N15) at (152.8bp,234.0bp) [draw=black,ellipse] {sqr\_N15};
%	\node (N8) at (205.8bp,90.0bp) [draw=black,ellipse] {add\_N8};
%	\node (N9) at (360.8bp,306.0bp) [draw=black,ellipse] {sub\_N9};
%	\node (N1) at (205.8bp,378.0bp) [draw=black,ellipse] {I0\_N1};
%	\node (N2) at (33.797bp,378.0bp) [draw=black,ellipse] {I1\_N2};
%	\node (N3) at (119.8bp,378.0bp) [draw=black,ellipse] {I2\_N3};
%	\node (N4) at (291.8bp,378.0bp) [draw=black,ellipse] {I3\_N4};
%	\node (N5) at (377.8bp,378.0bp) [draw=black,ellipse] {I4\_N5};
%	\node (N6) at (50.797bp,306.0bp) [draw=black,ellipse] {sub\_N6};
%	\node (N7) at (358.8bp,234.0bp) [draw=black,ellipse] {sqr\_N7};
%	\draw [->] (N12) ..controls (87.034bp,208.13bp) and (106.51bp,194.76bp)  .. (N13);
%	\draw [->] (N5) ..controls (371.79bp,352.26bp) and (369.5bp,342.82bp)  .. (N9);
%	\draw [->] (N7) ..controls (323.79bp,208.49bp) and (304.58bp,195.05bp)  .. (N14);
%	\draw [->] (N1) ..controls (187.16bp,352.38bp) and (178.81bp,341.35bp)  .. (N11);
%	\draw [->] (N8) ..controls (205.8bp,63.983bp) and (205.8bp,54.712bp)  .. (N17);
%	\draw [->] (N16) ..controls (258.8bp,207.98bp) and (258.8bp,198.71bp)  .. (N14);
%	\draw [->] (N15) ..controls (152.8bp,207.98bp) and (152.8bp,198.71bp)  .. (N13);
%	\draw [->] (N13) ..controls (171.89bp,135.78bp) and (180.01bp,125.06bp)  .. (N8);
%	\draw [->] (N1) ..controls (155.6bp,354.33bp) and (116.15bp,336.51bp)  .. (N6);
%	\draw [->] (N10) ..controls (258.8bp,279.98bp) and (258.8bp,270.71bp)  .. (N16);
%	\draw [->] (N4) ..controls (280.13bp,352.25bp) and (275.4bp,342.22bp)  .. (N10);
%	\draw [->] (N3) ..controls (131.47bp,352.25bp) and (136.19bp,342.22bp)  .. (N11);
%	\draw [->] (N2) ..controls (39.805bp,352.26bp) and (42.097bp,342.82bp)  .. (N6);
%	\draw [->] (N6) ..controls (50.797bp,279.98bp) and (50.797bp,270.71bp)  .. (N12);
%	\draw [->] (N1) ..controls (224.44bp,352.38bp) and (232.79bp,341.35bp)  .. (N10);
%	\draw [->] (N11) ..controls (152.8bp,279.98bp) and (152.8bp,270.71bp)  .. (N15);
%	\draw [->] (N9) ..controls (360.08bp,279.98bp) and (359.82bp,270.71bp)  .. (N7);
%	\draw [->] (N14) ..controls (239.7bp,135.78bp) and (231.59bp,125.06bp)  .. (N8);
%	\draw [->] (N1) ..controls (256.0bp,354.33bp) and (295.44bp,336.51bp)  .. (N9);
%	%	
%	\end{tikzpicture}
%	\label{dfg}
%	\hfill
%		%    \bottomrule
%	\end{tabular}
%\end{table}






%\begin{figure}[!h]
%	\centering
%
%\begin{lstlisting}[columns=fullflexible, language=C]
%#define SQR(x) ((x)*(x))
%for(int i=0;i<64;i++)
%	for(int j=1;j<63;j++)
%		for (int k=1;k<63;k++)
%			b[i][j][k] =
%				SQR(a[i][j][k] - a[i][j][k-1]) +
%				SQR(a[i][j][k] - a[i][j][k+1]) +
%				SQR(a[i][j][k] - a[i][j-1][k]) +
%				SQR(a[i][j][k] - a[i][j+1][k]);
%\end{lstlisting}
%	\caption{Application Program}
%	\label{code_app}
%\end{figure}
%
%
\begin{figure}[!h]
%	\captionsetup[subfigure]{justification=centering}
	\begin{subfigure}[fafsa]{}
	 % \begin{minipage}[t]{0.4\textwidth}
		\centering
		\begin{lstlisting}[columns=fullflexible, language=C, backgroundcolor=\color{white}]
		#define SQR(x) ((x)*(x))
		for(int i=0;i<64;i++)
			for(int j=1;j<63;j++)
				for (int k=1;k<63;k++)
					b[i][j][k] =
						SQR(a[i][j][k] - a[i][j][k-1]) +
						SQR(a[i][j][k] - a[i][j][k+1]) +
						SQR(a[i][j][k] - a[i][j-1][k]) +
						SQR(a[i][j][k] - a[i][j+1][k]);
		\end{lstlisting}
		        % \end{minipage}

		% \caption{Application Program}
		% \label{code}
	\end{subfigure}	


	\begin{subfigure}[dadad]{}
		\label{dfg}
	% \begin{minipage}[t]{0.44\textwidth}
	\centering	
	\begin{tikzpicture}[>=latex',line join=bevel, scale = 0.38]
	\centering	
	\tiny	
	\node (N12) at (50.797bp,234.0bp) [draw=black,ellipse] {sqr\_N10};
	\node (N13) at (152.8bp,162.0bp) [draw=black,ellipse] {add\_N14};
	\node (N10) at (258.8bp,306.0bp) [draw=black,ellipse] {sub\_N8};
	\node (N11) at (152.8bp,306.0bp) [draw=black,ellipse] {sub\_N7};
	\node (N16) at (258.8bp,234.0bp) [draw=black,ellipse] {sqr\_N12};
	\node (N17) at (205.8bp,18.0bp) [draw=black,ellipse] {O0\_N17};
	\node (N14) at (258.8bp,162.0bp) [draw=black,ellipse] {add\_N15};
	\node (N15) at (152.8bp,234.0bp) [draw=black,ellipse] {sqr\_N11};
	\node (N8) at (205.8bp,90.0bp) [draw=black,ellipse] {add\_N16};
	\node (N9) at (360.8bp,306.0bp) [draw=black,ellipse] {sub\_N9};
	\node (N1) at (205.8bp,378.0bp) [draw=black,ellipse] {I2\_N3};
	\node (N2) at (33.797bp,378.0bp) [draw=black,ellipse] {I0\_N1};
	\node (N3) at (119.8bp,378.0bp) [draw=black,ellipse] {I1\_N2};
	\node (N4) at (291.8bp,378.0bp) [draw=black,ellipse] {I3\_N4};
	\node (N5) at (377.8bp,378.0bp) [draw=black,ellipse] {I4\_N5};
	\node (N6) at (50.797bp,306.0bp) [draw=black,ellipse] {sub\_N6};
	\node (N7) at (358.8bp,234.0bp) [draw=black,ellipse] {sqr\_N13};
	\draw [->] (N12) ..controls (87.034bp,208.13bp) and (106.51bp,194.76bp)  .. (N13);
	\draw [->] (N5) ..controls (371.79bp,352.26bp) and (369.5bp,342.82bp)  .. (N9);
	\draw [->] (N7) ..controls (323.79bp,208.49bp) and (304.58bp,195.05bp)  .. (N14);
	\draw [->] (N1) ..controls (187.16bp,352.38bp) and (178.81bp,341.35bp)  .. (N11);
	\draw [->] (N8) ..controls (205.8bp,63.983bp) and (205.8bp,54.712bp)  .. (N17);
	\draw [->] (N16) ..controls (258.8bp,207.98bp) and (258.8bp,198.71bp)  .. (N14);
	\draw [->] (N15) ..controls (152.8bp,207.98bp) and (152.8bp,198.71bp)  .. (N13);
	\draw [->] (N13) ..controls (171.89bp,135.78bp) and (180.01bp,125.06bp)  .. (N8);
	\draw [->] (N1) ..controls (155.6bp,354.33bp) and (116.15bp,336.51bp)  .. (N6);
	\draw [->] (N10) ..controls (258.8bp,279.98bp) and (258.8bp,270.71bp)  .. (N16);
	\draw [->] (N4) ..controls (280.13bp,352.25bp) and (275.4bp,342.22bp)  .. (N10);
	\draw [->] (N3) ..controls (131.47bp,352.25bp) and (136.19bp,342.22bp)  .. (N11);
	\draw [->] (N2) ..controls (39.805bp,352.26bp) and (42.097bp,342.82bp)  .. (N6);
	\draw [->] (N6) ..controls (50.797bp,279.98bp) and (50.797bp,270.71bp)  .. (N12);
	\draw [->] (N1) ..controls (224.44bp,352.38bp) and (232.79bp,341.35bp)  .. (N10);
	\draw [->] (N11) ..controls (152.8bp,279.98bp) and (152.8bp,270.71bp)  .. (N15);
	\draw [->] (N9) ..controls (360.08bp,279.98bp) and (359.82bp,270.71bp)  .. (N7);
	\draw [->] (N14) ..controls (239.7bp,135.78bp) and (231.59bp,125.06bp)  .. (N8);
	\draw [->] (N1) ..controls (256.0bp,354.33bp) and (295.44bp,336.51bp)  .. (N9);	
	\end{tikzpicture}
	% \subcaption{A diagram}
			        % \end{minipage}
	\end{subfigure}

	% \caption{(a) Application Program (b) Data Flow Graph}
	\label{dfgs}
\end{figure}
%
%
%\begin{figure}[!h]
%	\centering
%%	\subfigure[Input DFG]{
%%		\centering
%\begin{lstlisting}[columns=fullflexible, language=C]
%#define SQR(x) ((x)*(x))
%for(int i=0;i<64;i++)
%	for(int j=1;j<63;j++)
%		for (int k=1;k<63;k++)
%			b[i][j][k] =
%				SQR(a[i][j][k] - a[i][j][k-1]) +
%				SQR(a[i][j][k] - a[i][j][k+1]) +
%				SQR(a[i][j][k] - a[i][j-1][k]) +
%				SQR(a[i][j][k] - a[i][j+1][k]);
%\end{lstlisting}
%\caption{Application Program}
%\label{code_app}
%		
%%	}
%	\hfill
%	\subfigure[Node-merging]{
%		\centering
%		\begin{tikzpicture}[>=latex',line join=bevel, scale = 0.3]
%		\tiny%
%		\node (N8) at (92.0bp,124.5bp) [draw=black,ellipse] {add\_Imm\_5\_N8};
%		\node (N9) at (46.0bp,10.5bp) [draw=black,ellipse,fill=red!20] {O0\_N9};
%		\node (N1) at (112.0bp,466.5bp) [draw=black,ellipse,fill=red!20] {I0\_N1};
%		\node (N2) at (46.0bp,67.5bp) [draw=black,ellipse,fill=red!20] {mul\_N2};
%		\node (N3) at (102.0bp,238.5bp) [draw=black,ellipse,fill=red!20] {mul\_N3};
%		\node (N4) at (112.0bp,409.5bp) [draw=black,ellipse,fill=red!20] {mul\_Imm\_16\_N4};
%		\node (N5) at (112.0bp,352.5bp) [draw=black,ellipse] {mul\_N5};
%		\node (N6) at (102.0bp,181.5bp) [draw=black,ellipse] {mul\_N6};
%		\node (N7) at (112.0bp,295.5bp) [draw=black,ellipse] {sub\_Imm\_20\_N7};
%		\draw [->] (N1) ..controls (146.27bp,446.62bp) and (178.55bp,423.54bp)  .. (167.0bp,399.0bp) .. controls (160.57bp,385.33bp) and (147.79bp,374.36bp)  .. (N5);
%		\draw [->] (N1) ..controls (159.02bp,444.04bp) and (224.0bp,407.12bp)  .. (224.0bp,353.5bp) .. controls (224.0bp,353.5bp) and (224.0bp,353.5bp)  .. (224.0bp,294.5bp) .. controls (224.0bp,243.78bp) and (166.06bp,209.78bp)  .. (N6);
%		\draw [->] (N3) ..controls (102.0bp,220.91bp) and (102.0bp,211.14bp)  .. (N6);
%		\draw [->] (N4) ..controls (112.0bp,391.91bp) and (112.0bp,382.14bp)  .. (N5);
%		\draw [->] (N5) ..controls (112.0bp,334.91bp) and (112.0bp,325.14bp)  .. (N7);
%		\draw [->] (N1) ..controls (64.984bp,444.04bp) and (0.0bp,407.12bp)  .. (0.0bp,353.5bp) .. controls (0.0bp,353.5bp) and (0.0bp,353.5bp)  .. (0.0bp,180.5bp) .. controls (0.0bp,144.98bp) and (20.045bp,107.55bp)  .. (N2);
%		\draw [->] (N7) ..controls (108.98bp,277.91bp) and (107.21bp,268.14bp)  .. (N3);
%		\draw [->] (N1) ..controls (84.093bp,450.73bp) and (65.284bp,437.6bp)  .. (57.0bp,420.0bp) .. controls (31.453bp,365.71bp) and (34.192bp,340.5bp)  .. (57.0bp,285.0bp) .. controls (62.03bp,272.76bp) and (72.121bp,262.06bp)  .. (N3);
%		\draw [->] (N8) ..controls (77.444bp,106.1bp) and (68.035bp,94.846bp)  .. (N2);
%		\draw [->] (N2) ..controls (46.0bp,49.908bp) and (46.0bp,40.144bp)  .. (N9);
%		\draw [->] (N1) ..controls (112.0bp,448.91bp) and (112.0bp,439.14bp)  .. (N4);
%		\draw [->] (N6) ..controls (98.983bp,163.91bp) and (97.208bp,154.14bp)  .. (N8);
%		%
%	
%		\end{tikzpicture}
%		\label{dfg_new}
%	}
%
%
%	
%	\caption[]{DSP48E1 aware mapping.}
%	\label{dfgs}
%	%\end{minipage}
%	
%\end{figure}

